Lord of LRDs: Insights into a "Little Red Dot" with a low-ionization spectrum at z = 0.1

Recent observations by the James Webb Space Telescope (JWST) have revealed a puzzling population of optically red and compact galaxies with peculiar "V"-shaped spectra at high redshift, known as "Little Red Dots" (LRDs). Until now, most spectroscopically confirmed LRDs are found at $z>4$ and it has been speculated that LRDs are tracing the early stages of black hole evolution. We report an independent rediscovery of a broad-line active galactic nucleus (AGN), SDSS J102530.29+140207.3, at $z=0.1$, which shows spectral features matching those of LRDs seen in the early Universe, including the V-shaped spectrum, broad Balmer lines (with widths of 1000-2000 km/s), and deep Balmer absorption. We present a new GTC observation of this LRD, which reveals an optical continuum similar to those of G-to-K giant stars including an unambiguous G-band absorption originating from the CH molecule. In addition, this local LRD shows a series of absorption lines potentially related to low-ionization ions or atoms but are deeper than what is observed in empirical stellar templates. We further identify a series of [FeII] emission lines indicative of low-ionization gas, which we find also present in a JWST-selected LRD at $z=2.26$. We find small but statistically significant variability in the H$\alpha$ of SDSS J102530.29+140207.3 consistent with previous findings. Finally, we report new observations with NuSTAR. We confirm the extreme X-ray weakness of this LRD, which might imply Compton-thick gas obscuration with $N_{\rm H}>10^{24}~{\rm cm^{-2}}$. All evidence suggests SDSS J102530.29+140207.3 has a complex gaseous environment and the strong ionic, atomic, and molecular absorptions are hard to explain with typical stellar and AGN models.

==> Tables/table_gmos.tex <==
\begin{table}
\centering
\caption{Bestf-fit parameters for the \ha\ emission and absorption as well as the NaD absorption assuming the broad \ha\ has an double-Gaussian profile.}\label{tab.gmos}
\begin{tabular}{ccc}
\hline
\hline
$\sigma_\mathrm{n}$ & $39.1_{-0.4}^{+0.4}$ & [\kms]       \\
$z_\mathrm{n}$  & $0.100501_{-0.000001}^{+0.000001}$ & [---]        \\
$F_\mathrm{n}(\mathrm{He\,I\lambda 5877})$ & $35_{-1}^{+2}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{[O\,I]\lambda 6300})$ & $15_{-1}^{+1}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\ha)$ & $856_{-7}^{+7}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{[N\,II]\lambda 6583})$ & $12_{-1}^{+1}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{He\,I\lambda 6679})$ & $10.0_{-1.0}^{+1.0}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{[S\,II]\lambda 6731})$ & $10.0_{-0.9}^{+0.8}$ & [\fluxcgs[-17][]] \\
$\mathrm{[SII]\lambda 6716}/\mathrm{[SII]\lambda 6731}$ & $1.1_{-0.1}^{+0.1}$ & [---]        \\
$F_\mathrm{n}(\mathrm{He\,I\lambda 7065})$ & $21.9_{-0.9}^{+1.0}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{[Ar\,III]\lambda 7138})$ & $8.4_{-0.9}^{+0.9}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{[Fe\,II]\lambda 7155})$ & $4.4_{-0.7}^{+0.7}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{[Ca\,II]\lambda 7291})$ & $10.1_{-0.7}^{+0.8}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{[Ca\,II]\lambda 7324})$ & $8.7_{-0.8}^{+0.9}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{n}(\mathrm{[O\,II]\lambda 7320})$ & $4.7_{-0.5}^{+0.6}$ & [\fluxcgs[-17][]] \\
$\mathrm{[OII]\lambda 7330}/\mathrm{[OII]\lambda 7320}$ & $0.51_{-0.04}^{+0.04}$ & [---]        \\
$v_\mathrm{b}$  & $3_{-1}^{+1}$ & [\kms]       \\
$F_\mathrm{b}(\ha)$ & $2640_{-10}^{+10}$ & [\fluxcgs[-17][]] \\
$F_\mathrm{b,1}/F_\mathrm{b}(\ha)$ & $0.416_{-0.007}^{+0.007}$ & [---]        \\
$FWHM_{\mathrm{b,1}}(\ha)$ & $727_{-10}^{+10}$ & [\kms]       \\
$FWHM_{\mathrm{b,2}}(\ha)$ & $2050_{-20}^{+20}$ & [\kms]       \\
$v_\mathrm{abs}$ & $-62_{-1}^{+1}$ & [\kms]       \\
$\sigma_\mathrm{abs}$ & $80_{-1}^{+1}$ & [\kms]       \\
$C_f$           & $0.85_{-0.02}^{+0.02}$ & [---]        \\
$\tau_0(\mathrm{\ha})$ & $3.3_{-0.3}^{+0.3}$ & [---]        \\
$v_\mathrm{Na\,I}$ & $-40_{-20}^{+20}$ & [\kms]       \\
$\sigma_\mathrm{Na\,I}$ & $110_{-20}^{+30}$ & [\kms]       \\
$C_{f,\mathrm{Na\,I}}$ & $0.47_{-0.05}^{+0.07}$ & [---]        \\
$\tau_0(\mathrm{Na\,I})$ & $2_{-1}^{+1}$ & [---]        \\
$EW_\mathrm{abs}(\ha)$ & $6.7_{-0.1}^{+0.1}$ & [\AA]        \\
$EW_\mathrm{cont}(\ha)$ & $5.73_{-0.09}^{+0.08}$ & [\AA]        \\
$EW_\mathrm{b}(\ha)$ & $-342_{-3}^{+2}$ & [\AA]        \\
$EW_\mathrm{abs}(\mathrm{Na\,I})$ & $13_{-1}^{+2}$ & [\AA]        \\
$EW_\mathrm{cont}(\mathrm{Na\,I})$ & $6.0_{-0.5}^{+0.6}$ & [\AA]        \\
$FWHM_{\mathrm{b}}(\ha)$ & $934_{-10}^{+10}$ & [\kms]       \\
$L_{\mathrm{n}}(\ha)$ & $0.234_{-0.002}^{+0.002}$ & [$10^{42} \rm{erg\,s^{-1}}$] \\
$L_{\mathrm{b}}(\ha)$ & $0.723_{-0.003}^{+0.003}$ & [$10^{42} \rm{erg\,s^{-1}}$] \\
$\log \mbh$   & $6.473_{-0.009}^{+0.009}$ & [dex \Msun]  \\
$\log SFR(\ha)$ & $-0.300_{-0.003}^{+0.003}$ & [dex \Msun yr$^{-1}$] \\
$\ledd$       & $0.252_{-0.006}^{+0.006}$ & [---]        \\
$\dot{M}_\mathrm{out,Na\,I}$ & $26_{-6}^{+10}$ & [\Msun yr$^{-1}$] \\

\hline
\end{tabular}

\raggedright{
Something wrong with EW NaI, possibly EW Ha too. The two EW NaI should be the same as a sanity check.}
\end{table}
